The Sensitivity of Language Models and Humans to Winograd Schema Perturbations

Large-scale pretrained language models are the major driving force behind recent improvements in performance on the Winograd Schema Challenge, a widely employed test of common sense reasoning ability. We show, however, with a new diagnostic dataset, that these models are sensitive to linguistic perturbations of the Winograd examples that minimally affect human understanding. Our results highlight interesting differences between humans and language models: language models are more sensitive to number or gender alternations and synonym replacements than humans, and humans are more stable and consistent in their predictions, maintain a much higher absolute performance, and perform better on non-associative instances than associative ones. Overall, humans are correct more often than out-of-the-box models, and the models are sometimes right for the wrong reasons. Finally, we show that fine-tuning on a large, task-specific dataset can offer a solution to these issues.

==> attention.tex <==
\section{On attention as an explanation}
\label{app:attn}


\subsection{Attention}
In this appendix, we provide an analysis of the attention mechanism of one of our models. There has been a large volume of work discussing whether, and to what extent, attention acts as an explanation for a network's decisions. We attempt to analyse the attention mechanism of our network to determine to what extent this is true.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{img/attn.png}
    \caption{Differences between attention weights for correct and incorrect referents; clusters are visible in the upper-right hand corner. Note the limited range expressed by the colourbar.}
    \label{fig:attn_map}
\end{figure}

Figure~\ref{fig:attn_map} is a map of the difference between the attention paid by the ambiguous pronoun to the correct and the incorrect referents. Several patterns do stand out -- in particular, there appear to be a few layer/head combinations that are `more active' than others. Further, as we would expect, the bulk of the weight appears to be concentrated towards the upper layers. It is crucial, however, to point out that the scale of this heatmap means that no matter how much these weights appear to stand out, they are still relatively small numbers, and their relatively low magnitude is compounded by the fact that these are the weights for the attention paid by only one element of the text to another.

To form a better picture of how attention weights specifically affect our system's prediction, we begin progressively masking heads, until all 16 heads are masked. Our heuristics for determining what word to mask depend on the attention paid to critical tokens. Based on these heuristics, we choose to either mask heads in both increasing and decreasing orders of importance. We also add an experiment masking a random head every iteration.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/mask.png}
    \caption{Drops in accuracy against the incremental masking of heads; heads are selected based on the attention paid to specific tokens (\emph{type}).}
    \label{fig:trendcols}
\end{figure*}

Figure~\ref{fig:trendcols} allows us to examine the drop in performance as the number of heads being masked increases. Interestingly, the results do \emph{not} appear to vary very strongly for the three masking directions, something we would expect if our predictions were strongly represented in our attention weights. The only outlier appears to be the attention paid to all non-critical tokens -- which, counterintuitively, leads to the sharpest decline in performance when heads are masked from most to least important. 

Finally, in Figure~\ref{fig:common_class}, we plot relevant POS and morphological information for tokens that receive the largest average shift in attention across all examples, per layer/head, when perturbed, for a subset of our perturbations. \todo{tidy up image} Our results show that whilst lower layers seem to capture perturbation specific tokens (numbered/gendered nouns for the number/gender task), higher layers (that also see more drastic shifts in weight), seem to capture more generic closed-class tokens. We defer analysis of this phenomenon to a future work.

\begin{figure*}
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{img/syn_tokclass.png} 
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{img/number_tokclass.png} 
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{img/gender_tokclass.png} 
    \end{subfigure}%
    \caption{TODO: pretty this up}
    \label{fig:common_class}
\end{figure*}{}



